Mathematical modeling in full-field optical coherence elastography

We provide a mathematical analysis of and a numerical framework for full-field optical coherence elastography, which has unique features including micron-scale resolution, real-time processing, and non-invasive imaging. We develop a novel algorithm for transforming volumetric optical images before and after the mechanical solicitation of a sample with sub-cellular resolution into quantitative shear modulus distributions. This has the potential to improve sensitivities and specificities in the biological and clinical applications of optical coherence tomography.

==> figures/approx1erordre.tex <==
% This file was created by matlab2tikz v0.4.2.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 
\begin{tikzpicture}

\begin{axis}[%
width=4.1in,
height=3.80333333333333in,
axis on top,
scale only axis,
xmin=-0.00168350168350168,
xmax=1.0016835016835,
ymin=-0.00168350168350168,
ymax=1.0016835016835,
colormap/jet,
colorbar,
point meta min=-1.09895893734547,
point meta max=1.20337084543728
]
\addplot graphics [xmin=-0.00168350168350168,xmax=1.0016835016835,ymin=-0.00168350168350168,ymax=1.0016835016835] {figures/approx1erordre-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/deltaeps.tex <==
% This file was created by matlab2tikz v0.4.2.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 
\begin{tikzpicture}

\begin{axis}[%
width=4.1in,
height=3.80333333333333in,
axis on top,
scale only axis,
xmin=-0.00168350168350168,
xmax=1.0016835016835,
ymin=-0.00168350168350168,
ymax=1.0016835016835,
colormap/jet,
colorbar,
point meta min=-2.99261184451044,
point meta max=2.77835138549722
]
\addplot graphics [xmin=-0.00168350168350168,xmax=1.0016835016835,ymin=-0.00168350168350168,ymax=1.0016835016835] {figures/deltaeps-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/epsilon.tex <==
% This file was created by matlab2tikz v0.4.2.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 
\begin{tikzpicture}[scale=0.6]

\begin{axis}[%
width=4.1in,
height=3.80333333333333in,
axis on top,
scale only axis,
xmin=-0.00167224080267559,
xmax=1.00167224080268,
ymin=-0.00167224080267559,
ymax=1.00167224080268,
colormap/jet,
colorbar,
point meta min=6.0676301430994,
point meta max=12.3250109564579
]
\addplot graphics [xmin=-0.00167224080267559,xmax=1.00167224080268,ymin=-0.00167224080267559,ymax=1.00167224080268] {figures/epsilon-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/mu_rec.tex <==
% This file was created by matlab2tikz v0.4.2.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
% 
% 
\begin{tikzpicture}

\begin{axis}[%
width=4.1in,
height=3.80333333333333in,
axis on top,
scale only axis,
xmin=-0.00167224080267559,
xmax=1.00167224080268,
ymin=-0.00167224080267559,
ymax=1.00167224080268,
colormap/jet,
colorbar,
point meta min=0.5,
point meta max=4.1518157320979
]
\addplot graphics [xmin=-0.00167224080267559,xmax=1.00167224080268,ymin=-0.00167224080267559,ymax=1.00167224080268] {figures/mu_rec-1.png};
\end{axis}
\end{tikzpicture}%
